Tube Formulae for Generalized von Koch Fractals through Scaling Functional Equations

In this work, we provide a treatment of scaling functional equations in a general setting involving fractals arising from sufficiently nice self-similar systems in order to analyze the tube functions, tube zeta functions, and complex dimensions of relative fractal drums. Namely, we express the volume of a tubular neighborhood in terms of scaled copies of itself and a remainder term and then solve this expression by means of the tube zeta functions. We then apply our methods to analyze these generalized von Koch fractals, which are a class of fractals that allow for different regular polygons and scaling ratios to be used in the construction of the standard von Koch curve and snowflake. In particular, we describe the volume of an inner tubular neighborhoods and the possible complex dimensions of such fractal snowflakes.

==> content/thmSetup.tex <==
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████
%
%           ██╗    ██╗██╗██╗     ██╗         ██╗  ██╗ ██████╗ ███████╗███████╗███████╗██████╗
%           ██║    ██║██║██║     ██║         ██║  ██║██╔═══██╗██╔════╝██╔════╝██╔════╝██╔══██╗
%           ██║ █╗ ██║██║██║     ██║         ███████║██║   ██║█████╗  █████╗  █████╗  ██████╔╝
%           ██║███╗██║██║██║     ██║         ██╔══██║██║   ██║██╔══╝  ██╔══╝  ██╔══╝  ██╔══██╗
%           ╚███╔███╔╝██║███████╗███████╗    ██║  ██║╚██████╔╝██║     ██║     ███████╗██║  ██║
%            ╚══╝╚══╝ ╚═╝╚══════╝╚══════╝    ╚═╝  ╚═╝ ╚═════╝ ╚═╝     ╚═╝     ╚══════╝╚═╝  ╚═╝
%
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████

\RequirePackage{mdframed, tikz}

% Theorems counter
\newcounter{theo}[section]
\numberwithin{theo}{section}

% Frame title settings
\newcommand{\frameTitleSetup}{
    \tikz[baseline=(current bounding box.east),outer sep=0pt]
    \node[anchor=east,rectangle,fill=blue!5,draw=blue,xshift=-20mm, inner ysep=2pt]
}

% Frame interior settings
\newcommand{\frameSetup}{
    \mdfsetup{
        innertopmargin=5pt,
        innerbottommargin=10pt,
        linecolor=blue,
        linewidth=1pt,
        topline=true,
        frametitleaboveskip=\dimexpr-\ht\strutbox\relax,
        frametitlealignment={\hspace*{0cm}},
    } 
}

% General environment setup
\newcommand{\envSetup}[2]{
    \newenvironment{#1}[1][]
    {%
        \refstepcounter{theo}%
        \mdfsetup{%
            frametitle={%
                \frameTitleSetup
                {\strut #2~\thetheo\ifstrempty{##1}{}{:~##1}};
            },
        }
        \frameSetup
        \begin{mdframed}[]\relax%
    }
    {\end{mdframed}}
}

% Create the environments for theorems, lemmas, etc.
\envSetup{theorem}{Theorem}
\envSetup{definition}{Definition}
\envSetup{lemma}{Lemma}
\envSetup{proposition}{Proposition}
\envSetup{corollary}{Corollary}

% Allow or disallow frames to split across page breaks
\mdfsetup{nobreak=true}


%████████████████████████████████████████████████████████████████████████████████████████████████████████████████
%█..............................................................................................................█
%█................................................................................**............................█
%█...........................................................................***********........................█
%█..........................................................................************........................█
%█............................................................................*********.........................█
%█..................................................................*....*.************..*......................█
%█..........................................................*****..*.**************************.................█
%█..........................................................***************************************.*****.......█
%█...........................................................*******************************************........█
%█.....................................................***.********************************************.*.......█
%█.......................................................*************************************************......█
%█..................................................********************************************************....█
%█...................................................*****************************************************......█
%█...........................***.*******.*..........*******************************************************.....█
%█...........................*****************.....*******************************************************......█
%█........................***********************.*********************************************************.....█
%█........................***********************.********************************************************......█
%█..................****.********************************************************************************.......█
%█**************************************************************************************************............█
%█..................****.********************************************************************************.......█
%█........................***********************.********************************************************......█
%█........................***********************.*********************************************************.....█
%█...........................*****************.....*******************************************************......█
%█...........................***.*******.*..........*******************************************************.....█
%█...................................................*****************************************************......█
%█..................................................********************************************************....█
%█......................................................*************************************************.......█
%█....................................................***.********************************************.*........█
%█..........................................................*******************************************.........█
%█.........................................................***************************************.*****........█
%█.........................................................*****..*.**************************..................█
%█.................................................................*....*.************..*.......................█
%█...........................................................................*********..........................█
%█.........................................................................************.........................█
%█..........................................................................***********.........................█
%█...............................................................................**.............................█
%█..............................................................................................................█
%████████████████████████████████████████████████████████████████████████████████████████████████████████████████

